Open- and Closed-Loop Neural Network Verification using Polynomial Zonotopes

We present a novel approach to efficiently compute tight non-convex enclosures of the image through neural networks with ReLU, sigmoid, or hyperbolic tangent activation functions. In particular, we abstract the input-output relation of each neuron by a polynomial approximation, which is evaluated in a set-based manner using polynomial zonotopes. While our approach can also can be beneficial for open-loop neural network verification, our main application is reachability analysis of neural network controlled systems, where polynomial zonotopes are able to capture the non-convexity caused by the neural network as well as the system dynamics. This results in a superior performance compared to other methods, as we demonstrate on various benchmarks.

==> figures/latexEquations <==
$\bigg \langle \begin{bmatrix} 4 \\ 0 \end{bmatrix},\begin{bmatrix} 1 & 0 \\ 0 & 2 \end{bmatrix},[~],\begin{bmatrix} 1 & 0 \\ 0 & 1 \end{bmatrix} \bigg \rangle_{PZ}$

$\bigg \langle \begin{bmatrix} 0 \\ 1 \end{bmatrix},\begin{bmatrix} 0.5 & -0.5 \\ 0 & 1 \end{bmatrix},[~],\begin{bmatrix} 1 & 0 \\ 0 & 1 \end{bmatrix} \bigg \rangle_{PZ}$

$\bigg \langle \begin{bmatrix} 1/8 \\ 1 \end{bmatrix},\begin{bmatrix} 1/4 & -1/4 & 1/16 & 1/16 & -1/8 \\ 0 & 1 & 0 & 0 & 0\end{bmatrix},\begin{bmatrix} 1/8 & 0 \\ 0 & 0 \end{bmatrix},\begin{bmatrix} 1 & 0 & 2 & 0 & 1 \\ 0 & 1 & 0 & 2 & 1\end{bmatrix} \bigg \rangle_{PZ}$

